ACETest: Automated Constraint Extraction for Testing Deep Learning Operators

Deep learning (DL) applications are prevalent nowadays as they can help with multiple tasks. DL libraries are essential for building DL applications. Furthermore, DL operators are the important building blocks of the DL libraries, that compute the multi-dimensional data (tensors). Therefore, bugs in DL operators can have great impacts. Testing is a practical approach for detecting bugs in DL operators. In order to test DL operators effectively, it is essential that the test cases pass the input validity check and are able to reach the core function logic of the operators. Hence, extracting the input validation constraints is required for generating high-quality test cases. Existing techniques rely on either human effort or documentation of DL library APIs to extract the constraints. They cannot extract complex constraints and the extracted constraints may differ from the actual code implementation. To address the challenge, we propose ACETest, a technique to automatically extract input validation constraints from the code to build valid yet diverse test cases which can effectively unveil bugs in the core function logic of DL operators. For this purpose, ACETest can automatically identify the input validation code in DL operators, extract the related constraints and generate test cases according to the constraints. The experimental results on popular DL libraries, TensorFlow and PyTorch, demonstrate that ACETest can extract constraints with higher quality than state-of-the-art (SOTA) techniques. Moreover, ACETest is capable of extracting 96.4% more constraints and detecting 1.95 to 55 times more bugs than SOTA techniques. In total, we have used ACETest to detect 108 previously unknown bugs on TensorFlow and PyTorch, with 87 of them confirmed by the developers. Lastly, five of the bugs were assigned with CVE IDs due to their security impacts.

==> approach-deprecated.tex <==
\section{Approach}



\subsection{Preprocessing}
Preliminary knowledge such as name, argument list, source code location, and corresponding low-level python API of DL operators is needed in further steps. DL operators are usually implemented as a class or a function sharing no common patterns in their names. It would be unrealistic to distinguish them from thousands of functions and classes. 

Fortunately, in most DL libraries, for high-level clients' reference, the source classes or functions of DL operators have to be registered and bound to a name through a specified macro definition. DL operators' arguments lists are also declared in a well-formatted file. For example, in TensorFlow, all operators are registered through the macro definition $ REGISTER\_KERNEL\_BUILDER $. A Protocol Buffers~\cite{protobuf} named $ops.pbtxt$ declares all the operators and their argument lists. Similarly, PyTorch~\cite{PyTorch} registered its operators with a macro definition $ KERNEL $ and declares all the operators in a yaml file named as $native\_functions.yaml$.

Leveraging these registration items and declaration files, we extract the attributions mentioned above in a simple matching manner.

\subsection{Validate Path Extraction}
In this stage, we extract the validate paths in operators for further constraint extraction. Path explosion is the main challenge for this step. But our basic goal is to generate validate input that passes the input validation at an acceptable expense, which means we do not have to extract all paths in an operator. Instead, we only need to extract constraints from paths in input validation code. But it remains a problem to identify input validation code, we manage to address this problem by proposing an novel technique for identifying input validation code in DL operators. Furthermore, to increase the possibility of exploring more paths, we extract all validate paths in input validation code.

\subsubsection{Input Validation Path Identification}
In this step, we identify the input validation code to avoid path explosion in path extraction. In traditional software, input validation code and functional code are usually mixed up and not likely to find the boundary between them. We distinct the input validation code based on two observations for DL operator: 
(1) Input validation is always conducted before computational part in DL operators. DL operators in popular DL libraries usually support different devices such as Intel CPU, Nvidia GPU, AMD GPU, and TPU. To maximize the use of hardware resources, device-specified computational code is implemented for various devices in most of the DL operators. It would be easier to validate input uniformly before entering separate computational code for different devices. 
(2) When the input validation fails, few specific functions are called. DL operators are usually executed in parallel as a part of DL models. A global execution context is used to manage multiple processes, few specific functions are used in all operators to notify the context validation fails.

Based on the observations, we manually conclude the name patterns of specific functions that indicate given input is invalid for target DL library. The input validation code in the target operator can be identified by traversing backward from calls to these functions to the entries in CFG(Control Flow Graph). The algorithm is shown in \algo ~\ref{alg:path_exp}.

\begin{algorithm} 
	\caption{Input validation code identification} 
	\label{alg:path_exp} 
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\begin{algorithmic}
		\REQUIRE $func\_patterns$, $ module $
		\STATE $cfg \leftarrow $.\textsc{build\_cfg}($module$)
		\STATE $bb\_set \leftarrow \{\}$
		\FOR{$func : $ \textsc{march\_funcs}($module$, $func\_patterns$)}
		    \FOR{$call\_site$ : $func.call\_sites$}
		        \STATE $bb\_set$.\textsc{add}(\textsc{backward\_dfs}($cfg$, $call\_site$))
		    \ENDFOR
		\ENDFOR
		\ENSURE  $bb\_set$
	\end{algorithmic} 
\end{algorithm}


\subsubsection{Path Extraction}
After identifying the boundary between the input validation code, the paths in input validation code are extracted in this step. The paths extracted are used for constraints extraction in the next stage. Technically, we have two options: (1) Extract paths lead to input invalidation exceptions, and generate input which violates the constraints in all of them. (2) Extract paths reach the boundary of input validation code without triggering any input validation exceptions, and then generate input satisfying constraints in each of them. 

The first strategy treats the valid input space as a whole. And the input is generated in the large space. However, the input space corresponding to some of the rare paths in the source code may be extremely small compared to the entire huge input space. Thus, most of the generated input may end up with exploring only one path in the source code. To increase the possibility of exploring more paths and also rare paths, we implement the second strategy and generates input for each validate path.

% In this step, we explore all paths in the target DL operator. There exists two optional strategies: 1) find all paths leading to errors, and generate input which violates the constraints in all paths. 2) find all paths leading to the return site without going through any errors, and generate input which satisfies the constraints in one of the paths. The two strategies are shown in \red{listing}.

% Path explosion is the main challenge for path exploration. Usually, check code and errors are placed before computational code in operators. The first strategy seems to be less affected by path explosion, as we can traverse backwards from the errors to find all paths and thus avoid traversing heavy computational parts. However, the generated input in the first strategy is hopeless to explore hardly reached branches, as it generates input in the whole correct input space. In order to explore more paths in the test phase, we choose the second strategy and propose a path pruning technique and a function skipping technique to avoid path explosion. The enhanced strategy is shown in \red{listing}.

% \begin{lstlisting}[frame=tb, caption=Code snippet in one of TensorFlow's operators, captionpos=b, float, label=listing:bias_example, belowskip=-0.7\baselineskip]
%     int channel_dim;
%     if (data_format_ == FORMAT_NCHW) {
%       channel_dim = 1;
%     } else {
%       channel_dim = input.shape().dims() - 1; 
%     }
% \end{lstlisting}

% \textbf{Path pruning.}
% Most code in DL operators is for computing instead of checking arguments, and check code is all we need to traverse. Thus we can prune the computational code after the check code is finished when traversing. The problem is how to distinct the computational code from the checking code. Here, we define the checking code as follows: if the code can lead to one of the errors, then it belongs to the checking code. Otherwise, it belongs to the computational code. Thus, a backward traverse from each error to the entry of the operator is conducted at first. All the traversed basic blocks are marked as check blocks. Then a forward traverse from the entry is conducted to find the correct path. During the traverse, once an ongoing path meets an error, the current traverse will be terminated. Once an ongoing path meets an unmarked basic block, the current traverse will be terminated and added to the set of successful paths.

% \textbf{Function skipping.}
% In DL operators, some functions do not affect the constraints, for example, log functions. Traversing these uninteresting functions is a waste of time. To identify and skip these uninteresting functions, we implement an algorithm. First, we conduct a value-flow graph for the target DL operator. Then we traverse the graph from each argument, all the traversed functions will be marked as interesting. Additionally, some frequently used and complex functions which are apparently unrelated to constraints are marked as uninteresting manually. For example, the constructor and destructor of strings and tensors.
% All uninteresting functions will be skipped in later path exploration. 


\subsection{Constraint Extraction}
This stage aims at extracting the constraints from the paths extracted in the previous stage. Symbolic execution is a common solution for extracting constraints from source code or binaries. But, complex structures such as $Tensor$ are common in DL operators. The overhead of blindly symbolizing all parameters in DL operators would be unacceptable. Thus, to extract constraints from the given paths in DL operators in a light-weight manner, we propose a constraint inference framework. The framework identifies user-controllable parameters and construct constraints by tracking their usages and propagating the controllibility.


% Symbolic execution is a common solution for extracting constraints from source code or binaries. Existing symbolic execution engines such as KLEE~\cite{KLEE} and angr~\cite{angr}, have achieved great success in constraint extraction. But they are not suitable for extracting constraints in DL operators because of the following reasons. KLEE requires to modify the source code of the target program manually. There are more than 1000 DL operators in TensorFlow, thus it would be a lot of human efforts to extract constraints with KLEE. The other tool, angr, is designed for binaries. The effect of extracting from binaries is limited when compared with extracting from source code. The last but most important reason is that blindly symbolizing all fields of arguments is expensive. According to our knowledge, the most common type of argument, tensor, is very complex, and it is used to represent high-dimensional matrices. And in most cases, the concrete values of matrices in tensor are not checked. Symbolizing those unrelated values would be a waste of time. What's more, a heavy symbolic execution would also result in redundant constraints and increase the burden of the input generation stage. Thus, existing symbolic execution engines are not suitable for extracting constraints in DL operators. To improve the efficiency of constraint extraction for DL operators, we design a constraint inference framework to extract constraints in a single path. The framework is then implemented in a symbolic execution engine.

\subsubsection{Constraint Inference Framework}
The main idea of the framework is that only specified properties of arguments are involved with constraints. Properties and constraints are inferred with actions defined in the framework. The following three paragraphs introduce the constraint inference framework in three aspects: interesting properties, property inference, and constraint inference.

\textbf{(1) Interesting properties.}  For each type of arguments, we identify its usually checked properties as interesting properties. For example, the number of dims of a tensor is often checked, so it is an interesting property of tensors. The elements of tensors and single characters in strings are rarely checked, so they are uninteresting values. Table ~\ref{table:properties} shows all interesting properties for each type.
\begin{table*}[h]
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{|l|l|l|l|}
            \hline
            \textbf{Argument Type} & \textbf{Interesting Property} & \textbf{Property Type} & \textbf{Description} \\ 
            \hline
            \multirow{4}{*}{tensor} & $dtype$ & dtype & \multicolumn{1}{|m{7cm}|}{The data type of the tensor.} \\
            \cline{2-4}
            ~ & $ndim$ & int & \multicolumn{1}{|m{7cm}|}{The number of dims of the tensor, and the length of the tensor's shape.} \\ 
            \cline{2-4}
            ~ & $num\_element$ & int & \multicolumn{1}{|m{7cm}|}{The total number of elements in the tensor.} \\ 
            \cline{2-4}
            ~ & $shape$ & list of int & \multicolumn{1}{|m{7cm}|}{The shape of the tensor.} \\
            \hline
            \multirow{4}{*}{list} & $element\_type$ & type & \multicolumn{1}{|m{7cm}|}{The type of the list's elements.} \\
            \cline{2-4}
            ~ & $length$ & int & \multicolumn{1}{|m{7cm}|}{The length of the list.} \\
            \cline{2-4}
            ~ & $loop\_value$ & int & \multicolumn{1}{|m{7cm}|}{The iterator value of the list, used when it is checked in a loop with an iterator.} \\
            \cline{2-4}
            ~ & $value$ & list of $element\_type$ & \multicolumn{1}{|m{7cm}|}{The concrete value of the list.} \\
            \hline
            \multirow{2}{*}{string} & $value$ & string & \multicolumn{1}{|m{7cm}|}{The value of itself.} \\
            \cline{2-4}
            ~ & $format\_id$ & int & \multicolumn{1}{|m{7cm}|}{The format id of this string if it is a format string of tensors.} \\
            \hline
            int & $value$ & int & \multicolumn{1}{|m{7cm}|}{The value of itself.}\\
            \hline
            float & $value$ & float & \multicolumn{1}{|m{7cm}|}{The value of itself.}\\
            \hline
            bool & $value$ & bool & \multicolumn{1}{|m{7cm}|}{The value of itself.}\\
            \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Interesting properties of each argument type}
    \label{table:properties}
\end{table*}

\textbf{(2) Property inference.} In the beginning stage of constraint extraction, only arguments can be identified easily in a path. The interesting properties must be inferred from the actions applied on these arguments and other interesting properties. For example, by applying $GetShape$ to tensor $t$, we can inference the result is $t.shape$. The inference chain of type tensor is shown in figure ~\ref{fig:prop_inf}. Blue nodes in figure ~\ref{fig:prop_inf} represent properties that are of basic types, and the ends of the inference chain.

\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{pics/property_inf.png}
	\caption{Inference chain of type tensor.}
	\label{fig:prop_inf}
\end{figure}

\begin{lstlisting}[frame=tb, caption=Code snippet in one of TensorFlow's operators, captionpos=b, float, label=listing:bias_example, belowskip=-0.7\baselineskip]
    int channel_dim;
    if (data_format_ == FORMAT_NCHW) {
      channel_dim = 1;
    } else {
      channel_dim = input.shape().dims() - 1; 
    }
\end{lstlisting}

\textbf{(3) Constraint inference.} We divide all the constraints into three types: natural constraints, basic constraints, and high-level constraints. Natural constraints are inherent between the properties of an argument and must be satisfied all the time. For example, the following constraints are natural constraints of a tensor $t$:
$$ t.shape.length = t.ndim $$
$$ \prod_{i=0}^{shape.length}t.shape[i] = t.num\_element $$
Basic constraints are produced by executing actions on properties of basic types. For example, listing ~\ref{listing:bias_example} is a code snippet in TensorFlow's operator, $BiasOp$, from the code in the $else$ branch, we can infer the following constraint from the subtraction:
$$ channel\_dim = input.ndim - 1 $$
Furthermore, high-level constraints are produced by executing actions on properties of structured types. For example, it is common to compare if tensor $t_1$ and tensor $t_2$ have the same shape in DL operators, and the following constraints can be inferred from this action:
$$ t_1.ndim = t_2.ndim $$
$$ t_1.shape[i] = t_2.shape[i], i=0,1,...,ndim-1 $$

By defining interesting properties, property inference rules and constraint inference rules, the constraint inference framework is able to extract constraints from paths in a light-weight manner.

\subsubsection{Symbolic Execution Engine}
The constraint inference framework is implemented in a symbolic execution engine. The engine works on the LLVM bitcodes of DL operators  based on SVF~\cite{SVF} and z3~\cite{z3}. SVF is used for constructing value-flow graph and z3 is used for constraints construction and solving. The paths collected in the path exploration stage are fed to the engine and satisfiable constraints of the paths are output. 

The engine is light-weight because it tracks only interesting values and translates interesting instructions. At first, only values of DL operators' arguments are marked as interesting. Then the engine traverses from the first instruction to the last instruction in each path. An instruction is interesting if all its operators are interesting or constant. Interesting instructions are translated in regards of their types.

\textbf{Arithmetic and logic instructions.} Each arithmetic and logic can be mapped into an action with the same semantic, which constructs a new constraint and marks the result value of the instruction as interesting. Typical instructions in this type include $add$, $sub$, $or$, $and$, $cmp$, $switch$ etc.

\textbf{Conditional branch instructions.} Conditional branch instructions are translated as a specific action, which constructs a constraint on the branch condition. Depending on the taken branch, the condition value is constrained to $1$ or $0$. Once an interesting conditional branch instruction is translated, the satisfiability of existing constraints will be checked. The engine will stop translating current path if the constraints are unsatisfied.

\textbf{Addressing instructions.} To handle $store$, $load$, $gep$ and other addressing instructions on interesting values, a virtual memory is maintained to record the corresponding values in each address. 

\textbf{Call instructions.} Actually, each of the actions that construct high-level constraints is mapped to a set of functions in a specified DL framework. For call instructions that call these functions, corresponding actions are executed and the called functions are skipped. Otherwise, the called functions are translated normally.

Other instructions such as $ret$, $jmp$ have no effect on values or constraints, thus it is okay to neglect them. 

The translated sub-path of each unsatisfied path is stored, and if a new path contains the same unsatisfiable path, it is unsatisfiable too. Finally, save the set of constraints in a path if it is satisfiable. 

The algorithm of the symbolic execution engine is shown in algorithm ~\ref{alg:cons_inf}.

\begin{algorithm} 
	\caption{Constraint inference} 
	\label{alg:cons_inf} 
	\renewcommand{\algorithmicrequire}{\textbf{Input:}}
	\renewcommand{\algorithmicensure}{\textbf{Output:}}
	\begin{algorithmic}
		\REQUIRE $paths$, $args$
		\STATE $arg\_values \leftarrow \{\}$
		\STATE $sat\_constraints \leftarrow \{\}$
		\STATE $unsat\_paths \leftarrow \{\}$
		\FOR{$arg : args$}
    		\FOR{$value :\ $\textsc{find\_values}($arg$)}
    		    \STATE $arg\_values$.\textsc{ADD}($value$)
    		\ENDFOR
		\ENDFOR
		\FOR{$path$ : $paths$}
		    \STATE $inst \leftarrow path$.\textsc{begin}()
		    \STATE $interesting\_values \leftarrow arg\_values$
		    \STATE $constraints \leftarrow \{\}$
		    \IF{\textsc{contain\_subpath}($path$, $unsat\_paths$)}
		        \STATE \textbf{continue}
		    \ENDIF
    		\WHILE{$inst \neq null$}
    		    \IF{\textsc{is\_interesting}($ inst, interesting\_values$)}
    		        \STATE $ action \leftarrow $ \textsc{get\_action}($ inst $)
    		        \STATE \textsc{apply\_action}($ inst, interesting\_values ,constraints$)
    		        \IF{\textsc{is\_cond\_branch}($ inst $)}
    		            \IF{!\textsc{check\_sat}($ constraints $)}
    		                \STATE $unsat\_paths$.\textsc{add}(\textsc{subpath}($inst, path$))
    		                \STATE \textbf{break}
    		            \ENDIF
    		        \ENDIF
    		        \IF{\textsc{is\_call}($ inst $)}
    		            \STATE $ inst \leftarrow $\textsc{skip\_function}($path, inst$)
    		        \ELSE
    		            \STATE $ inst \leftarrow $\textsc{next\_inst}($path, inst$)
    		        \ENDIF
    		    \ELSE
    		        \STATE $ inst \leftarrow $\textsc{next\_inst}($path, inst$)
    		    \ENDIF
    		\ENDWHILE
    		\IF{$!inst$}
    		    \STATE $sat\_constraints$.\textsc{ADD}($constraints$)
    		\ENDIF
		\ENDFOR
		\ENSURE  $sat\_constraints$
	\end{algorithmic} 
\end{algorithm}

\subsection{Input Generation}
Constraints in each path are collected and saved in a SMTv2 script. With the help of SMTSampler, we can get evenly distributed solutions easily. Technically, there is no more constraints for the rest of properties. Thus, they can be generated in a layered order, as shown in \red{fig}. Finally, test cases are saved as python scripts that call the corresponding low-level API of the target operator.

\subsection{Test}
The generated python scripts are executed in different modes and crashes are recorded. According to our knowledge, testing DL libraries suffers a lot from the long time (3~5 seconds) of loading DL libraries. Thus, a test process is maintained in the whole test phase to reduce boot time. A new test process is issued only when the former test process crashes or is killed because of timeout.


==> eva-scratch.tex <==
 \textbf{Metrics.} To evaluate the quality of our extracted constraints, we study them in two dimensions:
\begin{itemize}
    \item Average Constraint Number of each Property(\textbf{ACNP}): ACNP demonstrates the number and diversity of the constraints by measuring the number of constrained properties in each type. For each type of property, we calculate the times it being constrained among all the corresponding type of parameters. 
    $$ ACNP(tensor.dtype) = \sum_{tensor\ p}^{p \in tensors} \frac{isConstrained(p.dtype)}{tensors.size} $$
    \item Average Size of Max Relevant Subset: ASMRS shows the complexity of constraints of each API. Two parameters are relevant if they are constrained by each other. Thus,
    the parameters in each API can be divided into a few relevant subsets according to the given constraints. ASMRS of constraints extracted by a tool is calculated with the equation:
        $$ ASMRS(cons)= \sum_{api}^{api \in cons.keys().size} \frac{cons.keys().size}{GetMRS(cons[api]).size} $$
    In the equation, $cons$ is a dictionary mapping each API to its corresponding constraints extracted by the tool. And $GetMRS$ is a function that get the max relevant subset of all parameters in the given API.
\end{itemize}
To evaluate the quality of test cases we execute the generated test cases with target framework, and obtain the quality in two aspects:
\begin{itemize}
    \item Pass rate: Pass rate evaluates ratio of generated test cases that can pass all input validation checks. And therefore demonstrates the validity of generated test cases. Pass rate of a test round for an API can be calculated with the following equation:
        $$ PassRate(api) =  \frac{api.validate\_cases.size()}{api.test_cases.size()}$$
    \item Branch coverage: Branch coverage is a traditional metric for measuring the quality of the test cases. It reveals the 
\end{itemize}

\begin{table}[!ht]
\caption{ACNP of constraints extracted by DocTer and \tool}
    \centering
    \label{table:ACNP}
    \renewcommand\arraystretch{1.35}
    \begin{adjustbox}{max width=0.48\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \hline

        \textbf{Parameter Number} & value & dtype & length & value & dtype & dim & shape & \\ \hline
        \textbf{DocTer} & 197 & 238 & 0 & 0 & 896 & 200 & 63 & 1594\\ \hline
        \textbf{\tool} & 324 & 251 & 174 & 70 & 1172 & 577 & 499 & 3067\\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table}
